Symbolic Reachability Analysis of B through ProB and LTSmin

We present a symbolic reachability analysis approach for B that can provide a significant speedup over traditional explicit state model checking. The symbolic analysis is implemented by linking ProB to LTSmin, a high-performance language independent model checker. The link is achieved via LTSmin's PINS interface, allowing ProB to benefit from LTSmin's analysis algorithms, while only writing a few hundred lines of glue-code, along with a bridge between ProB and C using ZeroMQ. ProB supports model checking of several formal specification languages such as B, Event-B, Z and TLA. Our experiments are based on a wide variety of B-Method and Event-B models to demonstrate the efficiency of the new link. Among the tested categories are state space generation and deadlock detection; but action detection and invariant checking are also feasible in principle. In many cases we observe speedups of several orders of magnitude. We also compare the results with other approaches for improving model checking, such as partial order reduction or symmetry reduction. We thus provide a new scalable, symbolic analysis algorithm for the B-Method and Event-B, along with a platform to integrate other model checking improvements via LTSmin in the future.

==> 03-background.tex <==
% !TEX root = main.tex
\section{Integrating the B Operational Semantics into LTSMin [TO DO: remove and move to 02]}
\label{sec:integrating} % Background is not the good title for this section


\todo[inline, color=red!40]{This will include information on the Matrices:
Combined Dependency Matrix, Read Matrix, May-write matrix, Must-write matrix
State label dependency matrix, Guard matrix, Next-update function
Update matrix.\cite{DBLP:conf/ictac/BlomP08}, \cite{DBLP:conf/hvc/MeijerKBP14}}


\todo[inline, color=red!40]{We'll need to mention how it differs for Event-B to the B-Method here because we are not introducing the Event-B method.}


\subsection{Read-Write Matrix}
\label{sec:background:rw-m}
For the integration with LTSMin, we need to compute various pieces of information:
\begin{itemize}
 \item which variables are read in the guard of an operation
 \item which variables are read in the action part of an operation
 \item which variables must be written by an (enabled) operation and which variables may be written.
\end{itemize}
For correctness, we need to ensure that this information corresponds to the LTSMin view on what a transition is.
Indeed, LTSMin has no concept of parameters for events.
Take for example the following B operation with parameter {\tt p}:

\begin{small}
  Activate(p) = \Bselect pc=1 $\wedge$ p $\in$ ready \Bthen active := active $\cup$ \{p\} \Bend
%\begin{verbatim}
%  Activate(p) = SELECT pc=1 & p:ready THEN active := active \/ {p} END
%\end{verbatim}
\end{small}

It would be incorrect to say that the operation Activate has the following read/write matrix:

\begin{tabular}{c|c|c|c}
Reads Guard & Reads Action & Must Write & May Write\\
\hline
\{ready,pc\} & \{active\} & \{active\} & $\emptyset$
\end{tabular}

Indeed, for LTSmin {\tt p $\in$ ready} is not a guard \textcolor{red}{since {\tt p} is a parameter}, but influences the effect of the transition action.
Hence, we have to conceptually rewrite the operation into the following (normal) form:

\begin{small}
  Activate = \Bselect pc=1 \Bthen\\
       $\hspace*{1cm}$      \Bany p \Bwhere p $\in$ ready \Bthen active := active $\cup$ \{p\} \Bend \Bend 
\end{small}

This leads to the following read-write matrix, with the view that the guard is only {\tt pc=1}:

\begin{tabular}{c|c|c|c}
Reads Guard & Reads Action & Must Write & May Write\\
\hline
\{pc\} & \{ready,active\} & \{active\} & $\emptyset$
\end{tabular}

Note that when the assignment within an operation is of the form \verb+f(X) := E+ then the operation should have a read dependency on the function {\tt f}.

%\subsection{Partial Order Reduction}
%\label{sec:background:por}
%
%\todo[inline, color=red!40]{Do Not Accord matrix, Guard Necessary Enabling Set matrix,
%Guard Necessary Disabling Set matrix, Do Not Left Accord matrix,
%Must Disable matrix, Must Enable matrix.}

\subsubsection{Running Example Read-Write Matrix} \ \\
For our example in~\fref{fig:Bexample} the corresponding is the read-write matrix is as follows:

\begin{tabular}{l|l|l|l|l}
Operation &	Reads Guard &	Reads Action	& Must Write	& May Write\\
\hline
{\tt Enter}	& \{cs,wait\}	& \{cs,wait\}	& \{cs,wait\}&	$\emptyset$\\
{\tt Exit}	&\{cs\}	&\{cs,finished\}&\{cs,finished\} &$\emptyset$	\\
{\tt Leave} &	$\emptyset$	& $\emptyset$&	\{cs\}	& $\emptyset$\\
{\tt CS\_Active} &	\{cs\}	& $\emptyset$ & $\emptyset$ &$\emptyset$	\\
{\tt Restart} &	\{finished\}	&\{finished,wait\}	&\{finished,wait\}	&$\emptyset$\\
\end{tabular}

%
%\subsection{Partitioned Interface to the Next-State function (\pins)}
%\label{sec:background:pins}
%

\subsection{Read Matrix}
\label{sec:background:r-m}

\subsection{May-Write Matrix}
\label{sec:background:may-wm}

\subsection{Must-Write Matrix}
\label{sec:background:must-wm}

\subsection{Guard Matrix}
\label{sec:background:g-m}

\subsection{Next-update function}
\label{sec:background:nuf}

%For MAXINT=1 we get 4 states; the state space constructed by ProB can be found in Figure~\ref{fig:Mutex1States}.
For each of the 4 states in~\fref{fig:Mutex1States} ProB would check in each state, whether each of the 5 operations is enabled; resulting in 20 next-state calls.
With LTSmin symbolic model checking only 12 next-state calls are made, as shown in the following table.
Legend: +: enabled, - disabled, R: not computed (reused previous call).

\begin{tabular}{l|l|l|l|l|l|l|l|l}
State & cs & wait & finished & {\tt Enter} & {\tt Exit} & {\tt Leave} & {\tt CS\_Active} & {\tt Restart}\\ 
\hline
1 & FALSE & 1 & 0 & + & R & R & R & -\\ 
2 & TRUE & 0 & 0 & - & + & + & + & -\\ 
3 & FALSE & 0 & 0 & - & - & R & - & R\\ 
4 & FALSE & 0 & 1 & R & - & R & R & +\\ 
\end{tabular}

Figure~\ref{fig:Mutex1Ops} shows for each operation except for {\tt Leave} the projected states
on which they are computed, and in the case they are enabled what the effect is of performing the operation.
Definition~\ref{def:read-independence} ensures that the projected state space shown in Figure~\ref{fig:Mutex1Ops}
 can be used to compute the effect of each of these operations for the {\bf entire} state space.
 
For these four operations in~\fref{fig:Mutex1Ops} the read/write sets are identical.
Leave is different, it writes to a variable that is not read and is thus slightly harder to visualise in the same manner.
Indeed, {\tt Leave} will be computed just once by our approach, as it requires no input state.

\todo[inline, color=red!40]{Do you mean this:

For these four operations in~\fref{fig:Mutex1Ops} the read/write sets are identical? or do you mean? For these four operations in~\fref{fig:Mutex1Ops} each of the write sets are subsets of the read sets? explain what is the significance of this?}


%\begin{figure}[tb]
%\centering
%\includegraphics[width=.7\textwidth]{figures/MutexSimple1States.pdf}
%\caption{Mutex Simple Statespace for MAXINT=1}
%\label{fig:Mutex1States}
%\end{figure}


Note: if we initialise {\tt wait} with 500, the state space has 251,002 states.
Runtime with ProB is 70 seconds, with LTSMin bridge 48 seconds and doing only 6012 next state calls.
The example does not have a lot of concurrency and uses only simple data structures (and thus the overhead
of the LTSMin bridge is more of a factor compared to the runtime of ProB for computing next states); other examples will show greater speedups.
But the purpose of this example is to illustrate the principles.



==> fragments/highlevelFlowTooling.tex <==
\begin{tikzpicture}[->,>=latex,font=\sffamily,every node/.style={minimum width=3cm,
					minimum height=8em,outer sep=0pt,draw=black,semithick}]

	\node at (0,2) (F3) {\ltsmin};

	\node at (5,2) (F4) {\prob Link Library};

	\node at (10,2) (F5) {\prob Prolog CLI};
	\node [minimum width=1cm,minimum height=1.5em,anchor=south] at (F5.south) (F6) {Extension};

	\path[every node/.style={font=\sffamily\small}]
		(1.45,3) edge [above] node[right] {1} (3.4,3)
		(3.4,1) edge [above] node[left] {4} (1.45,1)
		(6.6,3) edge [above] node[right] {2} (8.45,3)
		(8.45,1) edge [above] node[left] {3} (6.6,1);
\end{tikzpicture}
